Conical spacetimes and global hyperbolicity

Vickers and Wilson (see Ref. 25) have shown global hyperbolicity of the conical spacetime in the sense of well-posedness of the initial value problem for the wave equation in generalized functions. We add the aspect of metric splitting and preliminary thoughts on Cauchy hypersurfaces and causal curves.

==> gmakros.tex <==
%\newcommand{\1}[1]{\leavevmode\kern.1em%
%  \raise0.05ex\hbox{\large 1}%
%  \kern-.65em
%  \raise.4ex\hbox{\underline{\ \ }}
%  \lower0.45ex\hbox{\scriptsize $#1$}}


% Paragraphenzeichen, weil \S fuer Schwartz-Raum verwendet
\def\pg{\mathhexbox278}

% Ingredienzen fuer Berechnungen und Abschaetzungen:
\newcommand{\stackup}[2]{\mathop{#1}\limits^%
{\substack{#2\\ \downarrow}}}
\newcommand{\stackdown}[2]{\mathop{#1}\limits_%
{\substack{\uparrow\\ #2}}}



% classical (function) spaces
\newcommand{\Con}{\ensuremath{\mathcal{C}}}
\newcommand{\Conc}{\ensuremath{\mathcal{C}_{\text{c}}}}
\newcommand{\Cinf}{\ensuremath{\mathcal{C}^\infty}}
\newcommand{\Cinfc}{\ensuremath{\mathcal{C}^\infty_{\text{c}}}}
\newcommand{\D}{\ensuremath{\mathcal{D}}}
\newcommand{\G}{\ensuremath{\mathcal{G}}}
\renewcommand{\S}{\mathscr{S}}
\newcommand{\E}{\ensuremath{\mathscr{E}}}
\newcommand{\OM}{\ensuremath{{\mathcal O}_\mathrm{M}}}
\newcommand{\OMs}{\ensuremath{{\mathcal O}_\mathrm{M,s}}}
\newcommand{\OC}{\ensuremath{{\mathcal O}_\mathrm{C}}}
\newcommand{\Zin}{\ensuremath{C_*}}
\newcommand{\Zho}{\ensuremath{\dot{C}_*}}
\newcommand{\loc}{\ensuremath{\text{loc}}}

% number sets
\newcommand{\mb}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\N}{\mb{N}}
\newcommand{\Q}{\mb{Q}}
\newcommand{\R}{\mb{R}}
\newcommand{\C}{\mb{C}}
\newcommand{\Z}{\mb{Z}}


% specialdistributions
\newcommand{\vp}{\mathrm{vp}}
\newcommand{\sgn}{\mathop{\mathrm{sgn}}}

% microlocal analysis
%\newcommand{\lara}[1]{\langle #1 \rangle}
\newcommand{\WF}{\mathrm{WF}}
\newcommand{\singsupp}{\mathrm{sing supp}}
\newcommand{\Char}{\ensuremath{\text{Char}}}
\newcommand{\zs}{\setminus 0}
\newcommand{\CO}{\ensuremath{T^*(\Om) \zs}}

% differential operators
\renewcommand{\d}{\ensuremath{\partial}}
\newcommand{\rd}{\ensuremath{\tilde{\partial}}} % regularized derivative
\newcommand{\diff}[1]{\frac{d}{d#1}}
\newcommand{\pdiff}[1]{\frac{\d}{\d#1}}
\newcommand{\der}[2]{\frac{d#1}{d#2}}
\newcommand{\pder}[2]{\frac{\d#1}{\d#2}}
\newcommand{\curl}{\mathop{\mathrm{curl}}}
\newcommand{\grad}{\mathop{\mathrm{grad}}}
\renewcommand{\div}{\mathop{\mathrm{div}}}
\newcommand{\jac}[1]{\mbox{D}#1}

% Fourier-Lebesgue measure
\newcommand{\dslash}{d\hspace{-0.4em}{ }^-\hspace{-0.2em}}

%     fonts and special characters
\newfont{\bl}{msbm10 scaled \magstep2}


% math environments
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
%  following commands are included in amsthm-package
%\newcommand{\qed}{\ \hfill$\square$}
%\newcommand{\proof}{{\sc proof:}\enspace}

% gue special comments
\newcommand{\hmm}[1]{($\triangleright$\ {\tt \small #1}\ $\triangleleft$)}
\newcommand{\todo}[1]{$\clubsuit$ \texttt{#1} $\clubsuit$}
\newcommand{\randbem}[1]{\marginpar{$\oslash${\small\texttt{#1}}}}
%\newcommand{\changed}{\marginpar{$\clubsuit$}}

% mappings
\newcommand{\map}{\ensuremath{\rightarrow}}
\newcommand{\emb}{\hookrightarrow}
\newcommand{\isom}{\cong}
\newcommand{\col}{\colon}
%\newcommand{\gto}{\mapsto}

%  transforms
\newcommand{\FT}[1]{\widehat{#1}}
%\newcommand{\Fg}[1]{\ensuremath{{\cal F}_{#1}}}
%\newcommand{\FS}{\Fg{S}}
\newcommand{\F}{\ensuremath{{\mathcal F}}}

% binary operators (bilinear ... et al)
\newcommand{\dis}[2]{\langle #1 , #2 \rangle}
\newcommand{\inp}[2]{\langle #1 | #2 \rangle}  %math mode
\newcommand{\notmid}{\mid\kern-0.5em\not\kern0.5em}
\newcommand{\egtd}{\stackrel{\mathrm{gtd}}{=}}
\newcommand{\ipsobolev}[3]{\langle #1|#2 \rangle_{#3}} %roland
\newcommand{\iphs}[2]{\langle #1 | #2 \rangle_{s}} %roland
\newcommand{\dishs}[2]{\dis{#1}{#2}_{H^{-s},H^s}}

% classical norms
\newcommand{\norm}[2]{{\| #1 \|}_{#2}}
\newcommand{\lone}[1]{\norm{#1}{L^1}}
\newcommand{\ltwo}[1]{\norm{#1}{L^2}}
\newcommand{\lp}[1]{\norm{#1}{L^p}}
\newcommand{\linf}[1]{\norm{#1}{L^\infty}}
\newcommand{\Zygnorm}[2]{\ensuremath{|#1|^*_{#2}}}
\newcommand{\Norm}[1]{\norm{#1}{}}
\newcommand{\nhs}[1]{\norm{#1}{H^s}} %roland
\newcommand{\nsobolev}[2]{\norm{#1}{H^{#2}}} %roland


% ancient greeks
\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\ga}{\gamma}
\newcommand{\Ga}{\Gamma}
\newcommand{\de}{\delta}
\newcommand{\eps}{\varepsilon}
\newcommand{\io}{\iota}
\newcommand{\vphi}{\varphi}
\newcommand{\ze}{\zeta}
\newcommand{\et}{\eta}
\newcommand{\la}{\lambda}
\newcommand{\La}{\Lambda}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}
\newcommand{\sig}{\sigma}
\newcommand{\Sig}{\Sigma}

% (linear) algebra
\newcommand{\inv}{^{-1}}
\newcommand{\trans}{{}^t}

% math lay-outs
\newcommand{\twocas}[2]{\left[\begin{array}{c}#1\\#2\end{array}\right]}

% misc
\newcommand{\supp}{\mathop{\mathrm{supp}}}
\newcommand{\floor}[1]{\ensuremath{\lfloor #1 \rfloor}}
\renewcommand{\Re}{\ensuremath{\mathop{\mathrm{Re}}}}
\renewcommand{\Im}{\ensuremath{\mathop{\mathrm{Im}}}}
\newcommand{\pa}{\partial}

% text lay-outs
%\renewcommand{\em}[1]{{\it #1\/}}
\newcommand{\ovl}[1]{\overline{#1}}
\newcommand{\jump}{\leavevmode\vspace{-1em}}



\newcommand{\ds}{\displaystyle}


%\DeclareMathOperator*{\add}{add}
%\DeclareMathOperator*{\Arg}{arg}
%\DeclareMathOperator*{\const}{const}
%\DeclareMathOperator*{\CONST}{const}
%\DeclareMathOperator*{\diam}{diam}
%\DeclareMathOperator*{\grad}{grad}
%\DeclareMathOperator*{\I}{I}
%\DeclareMathOperator*{\id}{id}
%\DeclareMathOperator*{\mult}{mult}
%\DeclareMathOperator*{\quot}{quot}
%\DeclareMathOperator*{\SPAN}{span}
%\DeclareMathOperator*{\rot}{rot}
%\DeclareMathOperator*{\vardiv}{div}

